Understanding and Auto-Adjusting Performance-Related Configurations

Modern software systems are often equipped with hundreds to thousands of configuration options, many of which greatly affect performance. Unfortunately, properly setting these configurations is challenging for developers due to the complex and dynamic nature of system workload and environment. In this paper, we first conduct an empirical study to understand performance-related configurations and the challenges of setting them in the real-world. Guided by our study, we design a systematic and general control-theoretic framework, SmartConf, to automatically set and dynamically adjust performance-related configurations to meet required operating constraints while optimizing other performance metrics. Evaluation shows that SmartConf is effective in solving real-world configuration problems, often providing better performance than even the best static configuration developers can choose under existing configuration systems.

==> tex/discussion.tex <==
\section{Disscussion} 
\label{sec:dis} 


%For example, both the RPC receiving queue size \texttt{ipcSize} in HB-3813 and the response queue size \texttt{responseSize} in HB-6728 can affect the memory significantly, and cause some fatal errors individually.  In Sec \ref{eval:hbase3813} and \ref{eval:hbase6728}, we demonstrate \tool outperforms static settings if we turn on each controller individually. However, without coordination, controller \texttt{ipcSize} and \texttt{responseSize} might increase at the sometime, so it is more likely to cause out of memory. This problem become much more serve when there are more controllers sharing the same performance goal, especially for no overshooting situation.

%For how to estimate the \textbf{needs}, the developers could potentially implement very complicated algorithm to estimate the demand. In our work, we only consider \textbf{needs} to be  1 or 0, which 1 stands for there is a demand, and 0 means there is no demand. For indirectly controller, there is a simple way to estimate the demand by considering the changes on passive controlled object \note{need a better terminology}. For example, in HBase3813, if current queue size is larger than previous queue size, this means \texttt{ipcSize} needs more a larger queue during this period. We can simply use this condition to estimate the \textbf{needs} for the controller using indirectly controller. During the experiment, we find out this simple rule has a good estimation of the \textbf{needs}. For directly control, we simply alway assume they have such \textbf{needs}, and set their corresponding \textbf{needs} as 1 \note{I do not have a better generalize solution for directly control, so I want to be somewhat conservative}. To coordinate different controller, we need to a central controller to suppress their increment if multiple controllers have the \textbf{needs} at the same time. We count how many controllers have the \textbf{needs} as $n$, and assign a equally weight of $\frac{1}{n}$ to these controllers. \revise{Specifically, instead of using $\frac{1-p}{\alpha}e_{k+1}$ for configuration update, we use  $\frac{1-p}{n\alpha}e_{k+1}$ in Eq. \ref{eq:controller}.} For those does not have the \textbf{needs}, the central controller won't suppress them. 
















==> tex/eval_raw.tex <==
\section{NOT NEEDED}
\subsection{HD-4995}
\subsubsection{Configuration Overview}

HDFS uses \texttt{dfs.content-summary.limit}, short for \texttt{limit}, to adjust the lock contention between the \texttt{du} command and the rest of the system. That is, \texttt{du} needs to hold a Namenode-system lock while traversing the file system. Since this lock is often highly contended, \texttt{du} releases this lock and acquires it again after traversing every \texttt{limit} number of files or directories.

%Specifically, if \textit{dfs.content-summary.limit} is too large, then the lock session could be very long, and potentially blocking many normal operations whatever needs this system level lock, like normal write requests. If this parameter is very small, it will cause frequently acquiring and releasing the lock, thus the overhead will slow down the \texttt{du} itself a lot. In this case, we consider worst write latency as the primary goal, since bug report mainly concerns about user level command like \texttt{du} should not block normal command for long time. Specifically, we consider the block level latency in our study. We consider the latency at block level since (1) this is more general, and we do not need to consider the size of individual write request and how it affect the performance, and (2) Hadoop Metric already considers such metric (WriteBlockOpAvgTime, Average time of write operations in milliseconds) at the Datanode level. Now we consider block level latency at Namenode, which is the actual end to end latency at server side. The second goal is to execution time of \texttt{du}, since we also want the user command does not take too much time.


In \hd{4995}, the user complains "it [du] could hold the namesystem lock for a long time ... 20 seconds ... should not allow regular users to cause extended locking.", as the default setting of \texttt{limit} is 0, essentially never releasing the lock.

%about the default \texttt{du} implementation will affect the system performance like normal write operation if the directory has too many directories and files. To reduce the tail latency of write request, the developer introduced a new functionality to allow the lock to be released and reacquire in middle when \texttt{du} is executed. Furthermore, they introduced a new configuration parameter \textit{dfs.content-summary.limit}. However, the developer disables this functionality by default. Our \tool automatically adjusts the configuration according to the current worst latency \wrt worst latency goal.

\subsubsection{Controller Synthesis} Following the user's complaint, our \texttt{limit} controller aims to minimize the \texttt{du} execution time while trying not to make the latency of those writes that execute concurrently with \texttt{du} too bad following a threshold specified by end users (e.g. 10 second)\shan{should we use write-throughput or request latency here?}. 

As shown in Table \ref{tab:evalbench}, \texttt{limit} \textit{indirectly} and \textit{conditionally} affects performance when \texttt{du} is executing by limiting the number of files \texttt{nFile} traversed in one critical section. Following this configuration property, we simply create a \texttt{SmartConf\_I} object for \texttt{limit} in HBase with the default transducer function, and invoke \texttt{getConf} exactly when \texttt{limit} is used in the original HBase. For performance sensing, we implement a function to measure block-level latency \shan{is your performance goal about per block?} at NameNode. In total, we made xx lines of code changes in HBase. 

\paragraph{Environment setting and profiling} 
We set up a HDFS cluster with xxxxx\shan{how many nodes, how many files and directories you are emulating blah blah}.
To build a model between  write-latency and \texttt{nFile} (the deputy of \texttt{limit}), we simply put 1GB File into HDFS cluster \shan{what does this mean?} while "du" is executing. 

%using a widely used HDFS performance benchmarks TestDFSIO \cite{testdfsio}.
%\shan{emm, do you get a model of latency vs limit or latency vs the real critical section size?}\shan{emm, i hope your profiling workload is different from the evaluation workload}. We then synthesize the controller to adjust \texttt{limit} based on the difference between xxx and xxx. This controller and corresponding \texttt{limit} adjustment is triggered only when 

\begin{comment}
In order to integrate the \tool into HDFS 4995, we need to make following changes.
\begin{enumerate}
\item HDFS 4995 does not provide write latency measurement at block level latency at Namenode\shan{why has to be at namenode? \revise{the lock is inside Namenode,and it is also true end to end latency at server side, from block creation to block finalization}}. We implement a sensor of block level latency at Namenode by obtaining the timestamps when a new block is allocated and when a block is finally finalized. Through matching the block ID information, we can obtain the block level latency by calculating the different between finish and start timestamps for the same block.
\item This parameter is used within \textit{getContentSummary()} function, so we invoke an update on this parameter before \textit{getContentSummary()} is called. 
\end{enumerate}
To integrate our controller based solution, we need to make XX lines code changes.
\end{comment}



\subsubsection{Experiment Results} 
To test how \tool works, we run the widely used HDFS performance benchmarks TestDFSIO \cite{testdfsio} on our HDFS cluster described above\shan{how is this benchmark different from your profiling workload?}. We start with a write-latency goal as 20 seconds, and then change the goal to 10 seconds during the execution. We will compare with two static configurations. 
\newline
\textbf{Controller solution V.S. Static Setting}: In the Fig. \ref{fig:hdfs4995basic}, initial worst latency is 168.5\% times larger than the initial goal 20s, and the controller reduces the configuration parameter based on the difference between worst latency goal and current worst latency. Once, the current write latency is round the performance goal, both primary goal and secondary goal are quite stable. For example, if we comparing with the static setting $10^8$ and dynamic solution we have. the overhead of our \tool in terms of du execution is around 25\% but has good ability to track the performance dynamically as well as reducing the worst latency by more than 2.5-5 times. A very small \textit{dfs.content-summary.limit} value like $10^5$ could reduce the worst latency significantly, but on the other hand, it causes an overhead on \texttt{du} execution time by 1.1 times.
\newline
\textbf{Controller solution under dynamic environment changes}: In the Fig. \ref{fig:hdfs4995basic}, we adjusts the performance goal at the runtime, and our \tool automatically tracks the goal like traditional feedback controller.

\begin{comment}
\begin{table}
	\centering
	\begin{tabular}{lrrrrccc}
		\toprule
		\textit{dcsl}	& $10^4$&  $10^5$ &  $10^6$ & $10^7$ &  $10^8$ &  $10^9$\\
		\midrule
		write latency(s) & 0.60 & 0.57 & 0.59 & 0.72 & 2.07 & \textbf{{\color{red}15.2}}\\ 
		\texttt{du} latency(s) & \textbf{{\color{red}243.0}} & 54.4 & 26.8 & 20.1 & 16.4 & 14.8\\
		\bottomrule
	\end{tabular}
	\caption{The different write and \texttt{du} latency under different \textit{dfs.content-summary.limit} (\textit{dcsl} for short) settings}
	\label{tab:hdfs4995tradeoff}
\end{table}
\end{comment}








\subsection{HB-3813}
\label{eval:hbase3813}
\subsubsection{Configuration Overview}: 
\textit{ipc.server.max.queue.size}, short for \texttt{ipcSize}, controls the maximum number of RPC calls appear inside a receiving queue inside the HRegionServer. The handler fetches these RPC calls from the receiving queue, and process their requests. This parameter plays an important role between memory usage and system performance. Specifically, if the queue size is large, then the memory consumption is large, thus more vulnerable to out of memory error; if the queue size is small, then it limits the RPC throughput at the server side.

\subsubsection{User Complaint:} The user explicitly complains about the default queue size is too large and "as possible cause of OOME(out of memory error)". The developers only change \texttt{ipcSize} to be configurable, and reduce the default queue size by 10 times in the patch. This developer also does not explore this configuration to default hbase configuration file \texttt{hbase-default.xml}.

%The developers only reduce the default queue size by 10 times in the patch. However, this patch does not fundamentally avoid the OOME if average request size is 10 times larger than that in their situation for example. Our \tool fundamentally solve this problem by dynamically adjusting queue size according to the current memory consumption \wrt memory limits.
\subsubsection{Controller Synthesis:} With \tool, we can build a \texttt{ipcSize} controller to maximize the request throughput while keeping used memory within heap limit.

From table \ref{tab:evalbench}, the \texttt{ipcSize} has a N-N-N setting for C-O-D property. It does not allow overshooting since violation on memory limit will cause fatal error, like server to be killed. This configuration only acts as proxy to limit the actually queue size.

We profile the HBase between actually queue size and \texttt{ipcSize}, along with some system properties. Then, \tool synthesize a no overshooting controller based on the profiling result we have. The controller adjusts \texttt{ipcSize} based on the difference between current used memory and memory limit. 

In order to leveraging \tool for this \texttt{ipcSize}, the developer needs to implement performance sensor for memory measurement (measure() function in SmartConf Class), which can be easily done by standard \textit{Java.lang.Runtime} class \textit{freeMemory()} and \textit{totalMemory()}. Then, the developer only need to place measure() and update() right before a new RPC call being putted into the receiving queue.


\begin{comment}
In order to integrate the controller into HBase 3183, we need to make following changes.
\begin{enumerate}
\item Since the source code from HBase 3183 does not allow to change the RPC callqueue online, so we need to change it to be dynamically tunable. For example, this can be done by either a large pre-allocated queue with additional queue size checking before putting RPC call into the queue or the solution suggested by developer in HBASE-15306. 
\item  We need a sensor to measure the heap usage inside HRegionServer, we can simply use standard \textit{Java.lang.Runtime} class \textit{freeMemory()} and \textit{totalMemory()} to obtain current used memory or reuse hbase metric library.
\item Before a new call being put into this queue, we invoke queue limit updates by supplying current queue size and current used heap memory, and max heap memory to the controller.
\end{enumerate}
To integrate controller based solution, we need to change XX lines code, which is easy for developer. We wrote a multi-threaded HBase Client, and sent write 1000 requests to the Hbase Server, with each request size is 1Mb. We use this workload for profiling to obtain the coefficient of system model $\alpha$, the pole $p_1$ and coefficient of variance $\lambda$ as we mentioned in Sec \ref{sec:controller_overshoot}, and the pole $p_2 =0$. 
\end{comment}
\subsubsection{Experiment Result:} We set up Pseudo-Distributed Hbase Cluster runing ontop of HDFS cluster with 5 replicas. For Hbase, we have one HMaster, HRegionServer and Zookeeper node. Each node with heap size of 512 MB. For the profiling workload, we use a multi-threaded HBase Client, and sent write 1000 requests to the Hbase Server, with each request size is 1Mb. For the testing, we consider two different workload, one is with 1Mb request size, another workload has request size of 2Mb.\note{I will update testing result using YCSB benchmark like others, this receiving is really about writing. Core workload focus more on reading request, might not suitable for testing. Could I use one write only or 50/50 read/write mix?}\shan{what does your question mean?} We comparing our \tool solution with two static configurations, one is queue limit equals 10, another is 200.
\newline
\textbf{Controller solution V.S. Static Setting}: In the Fig. \ref{fig:hbase3813basic}, \tool can utilize as much memory resource as possible, while withholding the used memory well below the memory limit (green line). The controller pulls back the queue limit once current used memory violates the virtual goal(purple line). If we use static configuration 200, HRegionServer will easily use up all the heap memory can cause OOME and crash the Server. If we limit the queue size too much, like 10, HRegionServer will not crash, but the RPC throughput much poor comparing with \tool, since it cannot full leveraging system memory resource. Specifically, in Throughput sub-Fig. \ref{fig:hbase3813basic}, the throughput of \tool is always high than static setting 10 and the final throughput performance is improved by 43.4\%. It is clear that \tool shows great advantage to keep the used memory from the memory violation and optimize the throughput as much as possible. The fundamental reason why \tool works better than static setting is controller takes current used memory \wrt memory limit into consideration, and then adjust the queue size accordingly.
\newline
\textbf{Controller solution under dynamic environment changes}: Since we consider the used memory in Java program, there are a lot of dynamic affected the used memory like garbage collection. Within each workload, the controller still function well, without any memory violation while maintaining high memory usage. Furthermore, to see how \tool deal with workload dynamic, we change the second workload with larger request size. Theoretically, if controller cannot properly deal with such workload changes but maintaining the same average queue size as before, it is very likely to cause OOME. However, from our experiment in third sub-Fig. \ref{fig:hbase3813basic}, the controller automatically reduced the queue size by roughly half, thus OOME does not happen. This means \tool is robust enough to deal with system dynamic, like workload changes, and fundamental reason is controller is operated based on current used memory rather than previous workload, and positive correlation between used memory and queue size is never changed.





\subsection{HB-6728}
\label{eval:hbase6728}
\subsubsection{Configuration Overview} Hbase uses configuration \texttt{ipc.server.response.queue.maxsize}, short for \texttt{responseSize},  to regulate the response queue size. The default setting is 1GB. Once current response queue occupies more than 1GB heap, it will block RPC Handler from putting new response into the response queue, which slows down requests throughput.

\subsubsection{User Complaint} A user complained that "This intermediate queue, because it has no bounds, can be another source of OOMs.". Therefore, the developer added a new functionality to throttle this response queue and a new configuration \texttt{responseSize} with a default value of 1GB. This configuration is hidden from the default Hbase configuration file \texttt{hbase-default.xml}, and only resides inside the source code. Although this problem is marked as major priority, there is no discussion or experiment on how to determine this value. It is obvious that this default value is useless if max JVM heap size is smaller than 1GB.

\subsubsection{Controller Synthesis} Our \texttt{responseSize} controller maximizes request throughput while keeping used memory within heap limit. 

From the table \ref{tab:evalbench}, the \texttt{responseSize} has a N-N-N setting for C-O-D property. It does not allow Overshoot, since violation on memory will cause fatal error like out of memory. This \texttt{responseSize} is a limit, which indirectly controls the actual response queue size.

Since \texttt{responseSize} is indirect control, we perform profiling between used memory and actual response queue size rather than response queue limit. Furthermore, the profiling also characterize the system property, which is useful for avoiding overshooting and suitable pole value. \tool automatically synthesize the controller to adjust the \texttt{responseSize} based on the difference between current used memory and memory limit. The update on \texttt{responseSize} happens whenever there is a new response is about to be putted into the response queue.

Similar to HBase 3813, the developer needs to implement performance sensor for memory measurement (measure() function in SmartConf class). Then, the developer need to insert measure() and update() before \texttt{responseSize} is used to stop inserting call into the queue, so that the \tool can obtain latest memory usage and adjust correspondingly.


\subsubsection{Experiment Result:} We use the same environment setting as HBase 3813. For the profiling workload, we use YCSB Workload A, with each record is 1Mb. We use two YCSB  Workload C (read only) and a 90/10 reads/write mix Workload for testing. We start with Workload C and then with mix Workload to better illustrate how controller reacts to the workload and environment changes. 
\newline
\textbf{Controller solution V.S. Static Setting}: We compare our solution with two static setting 10MB and 200MB. Under Workload C, the used memory under Static 200 MB is very close to the memory limits, and our controller well controls the used memory below the memory limits. Static 200 MB achieves the best throughput performance since it utilize more memory comparing with Static 10MB and Controller based solution. Later, we will see Static 200MB cannot handle system dynamic at all, and cause a huge fatal error. Although controller is more conservative than static 200MB, it is still better than static 10MB. 
\newline
\textbf{Controller solution under dynamic environment changes}: H After switching to mix read/write workload, the write requests start to occupy receiving RPC queue, which consumes the memory at the same time. Static 200MB does not aware the changes on workloads affects used memory, and finally cause out of memory error and killed the HRegionServer. On the contact, our controller based solution realized such changes through online used memory measurement, and it automatically limits Response queue size in the second workload as showed in Fig.\ref{fig:hbase6728basic}.    



\paragraph{Multiple controllers}
We also evaluated having both Hbase-3813 controller and Hbase-6728 controller active. We start with Put requests workload to write large amount data to Hbase, which consumes a lot memory inside RPC queue. After 50 second, we add other Get requests workload to obtain a amount large records from Hbase, and these Get requests are quite small when they are in receiving queue even they increase the RPC queue size a lot. However, when these Get requests are processed, each of them will have a large record for payload, and waiting inside the response queue to be sent back to client. The central realize such the \textbf{needs} changes for these two queues, and allowing response queue to increase, while keeping the whole memory well below the memory limits.
\note{Is there better experiment I should try? }






\subsection{HB-2149}
\subsubsection{Configuration Overview} 
HBase uses a pair of configurations \texttt{regionserver.global.memstore.upperLimit}
and \texttt{regionserver.global.memstore.lowerLimit}, 
short for \texttt{upperLimit} and \texttt{lowerLimit}, to regulate how much portion of the JVM heap could be occupied by the in-memory write cache \texttt{memstore}. The default setting is 40\% and 25\%. Once the \texttt{memstore} size reaches the \texttt{upperLimit} in a region server, its content gets flushed out to disk until reaching the a lower limit. All users' write requests are blocked during the flushing.

\subsubsection{User Complaint}
A user complained that ``The default value of \texttt{lowerLimit} of 25\% is too low ... very wrong ... problematic in almost all cases'', as flushing 15\% of the JVM heap could make ``ALL inserts blocked for 10-20 seconds or worse''. 
Developers acknowledged this problem and discussed whether the default value should be 0.35, 0.38, or almost 0.40. Concerned that making \texttt{lowerLimit} and \texttt{upperLimit} too close may cause too many small flushes and hence affect too many write requests, they settled down on ``a conservative value of 0.35'' without doing any experiments.

%although the worst latency of write request decreases,  the tail latency of write request actually becomes worse, because flush is triggered more frequently and more write requests are blocked by flush (Figure \ref{fig:2149-tradeoff}). This is a direct trade-offs between worst latency and tail latency of write requests. 

\subsubsection{Controller Synthesis}
Following the user's complaint, our \texttt{lowerLimit} controller aims to minimize the tail latency of write requests (e.g., xx\% percentile) while trying not to make the worst latency too large following a threshold specified by end users (e.g., 10 seconds in this user's complaint).\shan{may need to try another threshold and see what would happen. or at least comment on that.} 

As shown in Table \ref{tab:evalbench}, \texttt{lowerLimit} has a Y-Y-Y setting for the C-O-D property. It affects write latency directly but only during flushing (i.e., conditional); It allows Overshoot, as overshooting will not cause any system failures. 

Given this Y-Y-Y setting, we first obtain the write-latency--\texttt{lowerLimit} linear model by xxx. We then synthesize the controller to adjust \texttt{lowerLimit} based on the run-time difference between the worst latency and the threshold\shan{Sorry, did I change it wrong? is it the worst latency? is it the historically worst or worst in a recent time window?}. This controller and corresponding \texttt{lowerLimit} adjustment is triggered only when the flushing is ready to start. 

Overall, we changed xx lines of code in HBase.
xx lines of code is a new controller thread that implements our controller function\shan{do you have a common interface for the remaining system to invoke?}. With xx lines of code,
we modified \texttt{MemstoreFlusher} in HBase, so that \texttt{MemstoreFlusher} invokes our controller before every flushing. 
xx lines of code implements the sensor.
We modified each region server to send latency of each write request to the controller\shan{is each region server already measuring latency? on which node is the controller located? one on each RS? HMaster?}. Controller calculates the worst latency starting from the last region server level flushing event\shan{what does this sentence mean?}. \shan{maybe we can make this a table, so that we don't need to explain this much for each case repeatedly?}

\subsubsection{Experimental Results} 
We used YCSB Workload A \cite{ycsb} in our evaluation. It is a simulation of real-world write intensive workload, which contains 50\% reads and 50\% updates.\shan{can you briefly explain what this workload does? what is your HBase setting? What is your VM setting, unless the VM setting is explained somewhere else?} 

\textbf{Controller V.S. Static Setting}:
We compare our controller-adjusted \texttt{lowerLimit} with the static setting picked by developers in the patch (i.e., 0.35). This two setting delivers the same average latency -- xx vs. xxx\shan{please measure and present this}. Our controller setting provides much better tail performance, demonstrated by much less write requests taking more than 1 second to finish, as shown in Figure \ref{fig:2149-final}. \shan{1. make the tail the first figure; 2. change the curve to show percentage of requests over 1 sec?}
At the same time, our controller makes sure that the worse latency is around the threshold specified by the user.

\textbf{Controller under dynamic changes}:
To test how our controller would react to run-time changes, We changed the worst-latency threshold from 10 seconds to 6 seconds in the middle of the execution. As shown in Figure \ref{fig:2149-final}, once sensing the suddenly enlarged difference between actual worst write latency and the goal worst latency, controller quickly reacted by raising \textit{lowerLimit} from 0.15 to 0.25 to reduce the worst write latency. 

\shan{why does the static seems to finish all tasks earlier?}

\shan{i am a little bit concerned with this example. careless readers will very likely consider the worst latency result under controller to be BAD. in fact, when we set the threshold to be 10 seconds, the result seems to be as bad as what the original user complained about. isn't it?}
\begin{comment}
\begin{figure}
\centering
\includegraphics[width=2.5in]{fig/2149-tradeoff}
\caption{Cumulative distribution function of write request latency when \textit{lowerLimit} is 15\%, 25\%, and 35\%}
\label{fig:2149-tradeoff}
\end{figure}
\end{comment}




\subsection{CA-6059}
\subsubsection{Configuration Overview:}
Similar to HBase and other database system, when client writes data to Cassandra node, data will be first stored in \texttt{memtable}, in-memory write buffer in Cassandra. \textit{memtable\_total\_space\_in\_mb} (short for \textit{memtable\_total}) is a configuration that determines the maximum size of \texttt{memtable} in Cassandra.
\subsubsection{User Complaint:}
In Cassandra-6059, developers expressed that the current default value of \textit{memtable\_total}, which is one-third of JVM heap size, is "still too easy to OOM Cassandra even after moving sstable internals off heap". Thus, they reduced the default value to one-quarter of heap size. In this case, it is obvious that a larger \texttt{memtable} allows better write throughput and reduces the number of read cache miss by allocating a larger in-memory buffer. However, it also imposes a greater risk for Cassandra node to run out of memory, since more memory space may be used by \texttt{memtable}.

\subsubsection{Controller Synthesis:}
Based on the user's complaints, \textit{memtable\_total} tries to maximizes memory usage but ensures it never runs out of memory at the same time. 

\textit{memtable\_total} has a N-N-N setting for C-O-D property. \textit{memtable\_total} controls the maximum limit of size of \texttt{memtable} (indirect), which always affects memory usage; it does not allow overshooting, as out of memory will crash Cassandra node.

We measured the current memory usage of Cassandra node in Cassandra build-in class GCInspector, it will pass memory usage immediately after Garbage Collection to controller by calling controller's \texttt{measure(mem\_usage)} function.

\texttt{MemtablePool} class will invoke controller's \textit{update()} function to get updated \textit{memtable\_total} before it tries to put data into \texttt{memtable}. Controller will adjust new \textit{memtable\_total} based on current size of \texttt{memtable} (indirect) and the error between current memory usage and virtual goal (not allow overshooting).

\subsubsection{Experiment Result:} 
We set maximum heap size of Cassandra node to be 512MB, and we used YCSB workload A as our benchmark. 
\newline
\textbf{Controller solution V.S. Static Setting}:
We compared controller solution with two static settings, default setting after patch (\textit{memtable\_total} = 1/4 of heap) and a more aggressive setting (\textit{memtable\_total} = 1/2 of heap) in Figure \ref{fig:6059-result}. In the two YCSB workload A, controller used the most memory, and yielded best performance results. It finished two YCSB workload A faster than two static settings, as it used 240 seconds, conservative default setting used 310 seconds, and aggressive crash in the second workload. Figure \ref{fig:6059-result} demonstrated controller offered shorter read latency (it actually provided both shorter read and write latency). 
\newline
\textbf{Controller solution under dynamic environment changes}:
When the Cassandra finished the first workload, we added system dynamic by making Cassandra consume lots of heap memory, then we run the same workload again. (Chi: I increase memory usage by increasing the max read index limit from 5\% to 50\%, I am not sure whether mention it in paper, because I feel like it is very unusual) When \textit{memtable\_total} = 1/2 heap size, it run out of memory because of the sudden increase of memory usage. Although under the conservative setting, 1/4 of heap, it never run out of memory, but latency is almost twice of the other two runs. Controller reacted to the sudden memory usage burst by dropping \textit{memtable\_total} to guarantee not out of memory. Controller out-perform static setting by always guaranteeing memory usage is around virtual goal, which utilizes Cassandra heap memory and enabled better read and write performance.

\begin{comment}
\begin{figure}
\centering
\subfloat[Pole=0.5]{{\includegraphics[width=5cm]{fig/6059-oom-0_5} }}%
\subfloat[Pole=0.9]{{\includegraphics[width=5cm]{fig/6059-oom-0_9} }}%
\caption{Tune \textit{memtable\_total} at t+1 based on \textit{memtable\_total} at t}
\label{fig:6059-indirect}
\end{figure}
\end{comment}

\begin{comment}
\subsubsection{Experiment:}
The goal of controller solution is to control \textit{memtable\_total\_space\_in\_mb} so that it can utilize as much memory as possible without triggering OOM. In this case, the primary goal does not allow overshooting, and we used the virtual goal (). The controller can only tune \textit{memtable\_total}, which is the maximum size of \texttt{memtable}, rather than tuning the actual current size of \texttt{memtable} itself. In our experiment, when the used memory is below virtual goal, controller will try to increase \textit{memtable\_total}, but flush is usually triggered before \texttt{memtable} reaching maximum size, and current size of \texttt{memtable} is much smaller than \textit{memtable\_total}. As a result, controller keeps increasing \textit{memtable\_total}, until it is larger than heap size. It is quite dangerous to set \textit{memtable\_total} larger than heap size, because it will definitely trigger OOM, once there is a delay of flushing (Figure \ref{fig:6059-indirect}). We also tried using very large pole (0.9), but it still goes OOM. 

Instead, we used the technique introduced in Section \ref{sec:controller_indirect}, and control \textit{memtable\_total} based on current size of \texttt{memtable}. As shown in the Figure \ref{fig:6059-result}, this time, used memory size is guaranteed below JVM heap size and uses as much heap memory as possible to optimize read / write performance.
\end{comment}


\subsection{MR-2820}
\subsubsection{Configuration Overview}
MapReduce uses \texttt{mapred.local.dir.minspacestart}, short for \texttt{minspacestart}, to determine the minimum available space  before a tasktracker asks for a new task. In order to process a task, one needs to store intermediate files to disk whose size is varied depending on the workload. The insufficiency of free space leads to exception and fail the corresponding task. The intermediate file then will be cleaned up and the task will be rescheduled to another node. The failure of a task can induce the failure of the whole job once it fails for a configurable threshold.

In this particular problem, our objective is to minimize the job latency while keeping the number of exceptions in every tasks lower than the threshold. It can be accomplished by trying to process tasks as much as possible to increase job latency but stops when a task has failed for few times through increasing the \texttt{minspacestart}. Hence, the primary goal for the controller is to make the number of exceptions in every task lower than the threshold whereas the secondary goal is to improve the job latency. Since the controller cannot overshoot the primary goal, virtual target is needed. This configuration is directly and conditionally affects the performance. When the value is high, the exception is unlikely occurred, and vice versa. It also only takes effect when a node asked for a new task. 


\subsubsection{User Complaint}
A user complained that "the tasktracker still asked for a task even though the available disk space was less than 1\% as it caused the tasktracker to have a hard time to finish the tasks". Developer suggested to change the the \texttt{minspacestart} from the default value which is 0 to 1MB. However, it might not solved the problem since 1MB might be too small to be the threshold. An optimal \texttt{minspacestart} value is related to the workload due to the variation of the generated intermediate file size.





\subsubsection{Controller Synthesis}
\note{William: I will write this part according to the framework}
To sythesize the controller, profilling is done by trying several \textit{minspacestart} values and see whether it causes exception. \note{William: I am not so sure about my profilling since it is different from the others. Currently I use several (1, intermediate file size) pairs from a different split size and do a linear regression to it.}
The measure() function is triggered whenever a task is finished or failed. The performance is measured by calculating the current maximum number of exceptions in the unfinished tasks. It can be achieved by removing or adding a task's ID in a list when a task is finished or failed and calculate the maximum occurence of the IDs. The update() function is triggered whenever a task is finished or failed. The configuration value will be calculated using the measured performance and used by the tasktracker before it asks for a new task. The goal is specified by the failure threshold and virtual goal is needed. 

\subsubsection{Experimental Results}
We ran WordCount job to evaluate our controller which is one of the example jobs provided in Hadoop. The job reads a text file and counts each words occurrence. We use six virtual nodes with identical specification, one as a master and the others as slaves. The job was run in a three conditions with different values of \textit{mapred.max.split.size} (split size) and \textit{mapred.tasktracker.map.tasks.maximum} (parallelism number). We want to show that our controller can work even in different configuration setups. The different setups can affect the size of the generated intermediate file in a time which affect the optimal minspacestart value. In the first condition, we used both default values (64MB split size with 2 parallelism number) while in the second and third conditions, we change one of the default values to another value (64MB split size with 1 parallelism number and 128MB split size with 2 parallelism number). The \textit{mapred.map.max.attempts} which specifies the threshold of failures is set at 4 while the number of nodes with insufficient free space (200MB) is set at 4. 
\newline
\textbf{Controller solution V.S. Static Setting}:
Our controller-adjusted \texttt{minspacestart} is compared with the default static setting (0MB) and the all-around failure free static setting (230MB). As shown in the Figure 9, our controller provides generally better reliability and job latency, proved by the failure free execution and faster execution time. The controller manages to lower the current maximum number of exceptions when it exceeds the virtual target by increasing the minspacestart. The default static setting seems to struggle finishing the job whereas the failure free setting seems to have a bad execution time.     
\newline
\textbf{Controller solution under dynamic environment changes}:
We tested our controller with a few condition changes to check how our controller deals with it. Normally, when the value of split size or parallelism number is changed, the optimal minspacestart setting will also change. Our controller manages to compensate the difference and get a respectable result. 

\subsection{MR-5402}
In MR-5420, the user requested to make \textit{max\_chunks\_tolerable} constant configurable where he spotted a slow large workload with the default setting, which is 400. The constant defines the maximum number of created chunks that prohibit him to create more chunks to increase performance for the specific workload. This particular constant will only be used by DistCp, a default copying tool for large intra/inter cluster. It groups files into several chunks before being copied by a mapper. The number of chunks is affected by \textit{mapred.listing.split.ratio}, which determine the average number of chunks that will be processed by a mapper, and the number of mapper. 

We decided to set a goal to achieve the best execution time by predicting the \textit{mapred.listing.split.ratio} value. The goal could not be attained by the controller due to its limitation to always track the goal. Moreover, the relationship between the \textit{mapred.listing.split.ratio} and the execution time is not monotonic, making it harder to apply linear regression to get an approximation of how the system reacts to the control variable. The problem gets compounded by considering the pricey process of reshuffling chunks when we changed the split ratio in runtime.

(Should we include how I use machine learning to solve this problem e.g feature selectionn and determining a good algorithm by doing machine learning experiments, and the result of the predictor?)




==> tex/evalworkload_tab.tex <==
\begin{table*}[t]
\centering
%\begin{tabular}{lp{0.28\linewidth}p{0.28\linewidth} p{0.28\linewidth}}
{\footnotesize
\begin{tabular}{llllll}
	\toprule
ID	& Profiling Workload & \multicolumn{4}{c}{Evaluation Workload}\\
\cline{3-4}
\cline{5-6}
    &                    & Phase-1 Workload & Constraint & Phase-2 Workload & Constraints\\
	\midrule
    CA-6059 &YCSB$_A$ (1MB) &YCSB (0.9W,1MB,Cache0)&!OOM &YCSB (0.9W,1MB,Cache 0.5)&!OOM \\
    %CA-6059 &YCSB(0R/1W,1MB) &YCSB (0.5W/0.5,1MB,Cache 0) &YCSB (0.5R/0.5W,1MB,Cache 0.5) \\
    % HB-2149 might try default request size 1KB.
    HB-2149 &YCSB$_A$ (1MB) &YCSB (1.0W,1MB) & 10 sec &YCSB (1.0W,1MB) & 5 sec \\  
    HB-3813 &YCSB$_A$ (1MB) &YCSB (1.0W,1MB)&!OOM &YCSB (1.0W,2MB)&!OOM\\
    HB-6728 &YCSB$_A$ (1MB) &YCSB (0.0W,2MB) &!OOM&YCSB (0.3W,2MB)&!OOM\\
    HD-4995 &TestDFSIO$_{\text{single-thread}}\cite{huang2010hibench}$ &TestDFSIO$_{\text{multi-thread}}$& 10 sec& TestDFSIO$_{\text{multi-thread}}$ & 5 sec\\
    MR-2820 &Wordcount(2G,64MB,1) &Wordcount(640MB,64MB,2) &\#OOD<4&Wordcount(640MB,128MB,2) & \#OOD<4\\
        %\multirow{2}{*}{HB-3813} & YCSB (50\%read/ 50\%Write)  &  YCSB write-only & YCSB write-only \\
    %&Request size 1MB &Request size 1MB& Request size 2MB\\ 
    %\midrule
    %\multirow{2}{*}{HB-6728} & YCSB (50\%read/ 50\%Write)  &  YCSB read-only & YCSB (90\%read/ 10\%Write) \\
            %&Request size 1MB &Request size 2MB& Request size 2MB\\
    %\midrule
    %\multirow{2}{*}{HD-4995} & Single Thread TestDFSIO &  TestDFSIOEnh (multiple threaded)  & TestDFSIOEnh \\
            %& &Latency Goal 10s& Latency Goal 5s\\
    %\midrule
      %\multirow{2}{*}{HB-2149} & YCSB (50\%read/ 50\%Write)   &  YCSB write-only & YCSB write-only \\
            %&Request size 100KB &Request size 100KB& Request size 100KB and half heap is used by index cache\\
    %\midrule
 %\multirow{2}{*}{MR-2820} & a wordcount job to process a large file (2GB) &  a different file (640MB)  & a different file (640MB) \\
            %&default split size 64MB, 1 map parallelism, and 5 slaves node &Split size : 64MB, parallelism : 2& Split size : 128MB, parallelism : 2\\
	\bottomrule
\end{tabular}
}
\caption{Evaluation and profiling workload \textmd{(YCSB(xW,yMb): YCSB \cite{cooper2010benchmarking} workload with \textit{x} portion of write and request size of \textit{y}MB. Wordcount(x,y,z): x -- input file size; y -- split size; z -- parallelism per worker\shan{to revise})}}
\label{tab:workload}
\end{table*}


==> tex/fig.tex <==





\begin{figure}
\centering
\includegraphics[width=3in]{fig/hdfs4995basic}
\caption{HDFS 4995 controller based solution under goal changes}
\label{fig:hdfs4995basic}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=3in]{fig/hbase3813basic}
\caption{Hbase 3813 Control based solution Under workload changes around 200s}
\label{fig:hbase3813basic2}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=3in]{fig/hbase6728new}
\caption{Hbase 6728 Basic controller}
\label{fig:hbase6728basic}
\end{figure}


\begin{figure}
\centering
\includegraphics[width=3.5in]{fig/2149-final}
\caption{Example of figure template}
\label{fig:2149-final}
\end{figure}




\begin{figure}
\centering
\includegraphics[width=3.5in]{fig/6059-result}
\caption{Controller}
\label{fig:6059-result}
\end{figure}



\begin{figure}
\centering
\includegraphics[width=3.5in]{fig/MR2820}
\caption{Controller}
\label{fig:mr2820}
\end{figure}

==> tex/intro-old.tex <==
\section{Introduction}
\label{sec:intro}

\subsection{Motivation}
Modern software systems are increasing complicated, often
equipped with hundreds to thousands of configuration options allowing
customization. 
Unfortunately, users and developers cannot possibly set all of these configuration parameters appropriately, leading to 
mis-configuration as one of the biggest causes of system misbehavior
%, leading to almost 40\% of system
%downtime 
\cite{whypcstops,yy.sosp13,yimin}.
Mis-configuration leads to both functionality 
(e.g., wrong outputs, crashes) and performance problems.
Although the former has been tackled by much recent
research \cite{yy.sosp13,tianyin.acs}, the latter still remains an open
problem, becoming increasingly troublesome with the growing complexity of 
modern software systems, particularly server systems.
%TODO

%For example,
%Hadoop MapReduce, a widely used big-data programming infrastructure,
%contains about 500 configuration options; 
%Firefox browser has more than
%1000 configuration options.

In server applications, performance-sensitive configurations are common and
their settings severely affect server performance and availability. 
These configurations control the size of performance-critical data structures, 
the frequency of performance-sensitive operations, the thresholds and weights
in workload-dependent algorithms, and so on. Previous study has shown that 
xx\% of server configurations are related to performance. Meanwhile, improper
configuration settings can lead to integer multiple of performance
differences \cite{xx} and system downtime caused by excessive memory
usage (i.e., out-of-memory failures) or disk usage (i.e., out-of-disk failures).
\shan{Please check Xray paper, Duke paper, tianyin's paper to find out some
motivational citations, statistics.}

Unfortunately, properly setting performance-sensitive configurations is
challenging. The highest performance settings depend on
hardware, workload characteristics, and other factors.
Often times, the relationship between the former and the latter is not 
or cannot be clearly explained in the software documentation \cite{}. 
Even when the documentation is clear, 
the workload characteristics are often too complicated or change too
quickly for a user to maintain a proper setting \cite{}.
Even worse, sometimes, a job many contain multiple phases, each
demanding different configuration settings for a good performance. 
In this case, there simply exists no proper static setting \cite{itask}.

\hank{The next two paragraphs set up related work.  I feel like what is missing from this discussion is the notion that many of these parameters represent a tradeoff.  For example, queue size often represents a tradeoff between memory usage and response time (and we can back this up with data).  One of the reasons that setting the configurations parameters is so hard is that you have to navigate a tradeoff space; e.g., find the queue size that provides the lowest response time that does not cause the system to run out of memory.  Finding the best (e.g., lowest response time) configuration that meets a constraint (no out-of-memory errors) is a hard problem; harder than simply finding the fastest configuration.

Two major challenges in solving these constrained optimization problems in computer systems:
\begin{itemize}
\item The best configuration can change based on unpredictable, external events.  For example, a queue size that is safe in one instance, may not be when another part of the system unexpectedly allocates a large data structure.
\item The constraints in these systems are often safety critical, and thus cannot be violated.  For example, while it may cause use dissatisfaction to violate a response time constraint, violating a memory constraint will crash the system.
\end{itemize}

Prior work has addressed the problem of configuring software to meet constrained optimization problems in several ways:
\begin{itemize}
\item The industry standard is simply to expose parameters to users who are forced to become both application and system experts to understand the best settings for their particular hardware and workload. (Citations? Forward reference to bug study?)
\item Machine learning techniques can explore complex configurations spaces to find near optimal settings \cite{SomeMLStuff}. While ML approaches are good at finding optimal solutions to configurations problems, they are less well suited for managing constraints, especially in dynamic environments.
\item Control theory has been used to perform constrained optimization for \emph{non-functional} software properties; i.e., those that are not safety critical, like performance. Control theory has formal mechanisms for reasoning about software behavior in dynamic environments, but prior approaches are not well-suited to functional requirements; e.g., prevent out-of-memory errors.  
\end{itemize}
}

Several techniques tackle this problem.
One is to eliminate a specific performance-sensitive configuration through
a better algorithm. For example, instead of letting users to 
specify which job is interactive and which is not, a scheduling algorithm
can infer which job is interactive based on its run-time behavior. This approach can be very effective for certain cases. However, it only solves
one problem at a time. Furthermore, not all configurations can be 
eliminated.\shan{emm, maybe this is essentially about machine learning and building model?}

Another approach is to build a model through machine learning techniques
and a large amount of profiling. xx. This approach is effective for xx.
However, there are often many dynamic environment and workload fluctuation that can affect performance and invalidate
a prior-built model.
For example, it is unclear how much and what type of hardware-resource 
contention a job might get when it is running. xxx\shan{I am running out of my depth here :S}

%TODO Performance auto-tuning \cite{andy.pavlo}.
%TODO Klara group's prior work, and search auto-configuration



\subsection{Contributions}
In this paper, we first conduct an empirical study to understand
real-world performance-related configuration problems.
We then propose a control-theory based framework to help automatically
set performance-sensitive configurations. Unlike prior control theoretic work, our framework is specifically designed to handle safety-critical constraints; e.g., ensuring limits on memory consumption. 

%control-theory techniques to allow software to automatically adjust its
%own configurations, while achieving good performance and 
%quality of service guarantees.

Our empirical study covers 4 widely used open-source large scale systems (Cassandra, HBase, HDFS, and MapReduce). For these applications, we studied 100 developer-patches that make changes to performance-related configurations, as well as 100 user-posts that discuss performance-related configurations. 
Our study has answered several key questions to
guide future research on performance-related auto-configuration.
\begin{enumerate}
\item \emph{How important are performance related configuration problems?}
Even though performance impact is much harder to be perceived than functionality problems,
our study still finds that 40\% of configuration patches committed by developers 
introduce or change configurations for performance reasons;
25\% of configuration related user complaints are about performance issues\shan{numbers to be updated}.
These numbers indicate that properly setting performance-sensitive configurations
is a serious issue in the real world.
\item \emph{How does configuration affect performance?}
Real-world configurations affect a wide range of performance issues.
Among users' complaints, 
xx\% of them are about memory consumption (out of memory),
xx\% is about job turn-around time, xxx. 
For xx\% of the configurations, their impact to performance is conditional,
while the other ones impose always-on performance impact.
Many (xx\%) configurations do not directly affect performance, but they impose constraints to other system variables that directly affect performance.
Most (more than xx\%) configurations affect more than one major performance
metrics. Their impact to a performance metric is 
is mostly monotonic (xx\%), although almost never linear.

\item \emph{How to set performance-sensitive configurations?}
In our study,
xx\% of performance-sensitive configurations are numerical typed.
Properly setting xx\% of configurations require understanding of the
run-time workload; xx\% of them can benefit from run-time adjustment
that is not supported by software's existing configuration mechanism. 

\item \hank{Can we add something about the number of these bugs that represent constrained optimization problems (e.g. queue size is a tradeoff between response time and memory usage), because I would like to emphasize that our solution handles constrained optimization, and is not generally the best approach to a strict optimization problem.}
\end{enumerate}

\hank{What is below is very general, and maybe that is the right thing to do.  Is it worth adding something specific about what we are doing that separates us from prior control approaches?  At a high-level, I see our contribution over prior control approaches is designing a general framework that can still meet safety-critical constraints.  Prior work is either (1) general, but with no ability to handle safety critical constraints or (2) handles safety-critical constraints by building a system specific approach.  We get generality and safety by: (1) use of a virtual goal set based on the application's statistical profile and (2) use of a switching (or adaptive or context-aware) control sytsem that is conservative when in the safe region and aggressive if it ever enters an unsafe region (operating beyond the virtual goal).}
Guided by our empirical study, we explore a systematic and general
control-theoretic solution to automatically set and dynamically
adjust performance-sensitive configurations to meet required operating constraints while optimizing other behavior.

Facing a wide variety of controller design options, we carefully picked
the ones that are most suitable for real-world performance-sensitive
configurations guide by the empirical study above. 

We further identify unique challenges that are not handled by existing
control theory and design our own controller techniques to address these challenges. Specifically, we design new techniques to handle configurations that do not directly affect performance, and configurations whose performance requirements do not allow over-shooting the targets.

We then come up with a step-by-step recipe that helps developers to turn a 
configuration
from its traditional format (i.e., developers/users need to manually
set it) into automatically adjustable. Our recipe covers a wide variety of performance-related configurations by abstracting three key properties of performance-configuration issues and use them to customize a uniform work flow that consists of profiling, controller synthesis, sensor, controller invocation, and configuration updating.

Finally, we apply our recipe to solve real-world configuration problems
in widely used open-source distributed systems (Hadoop MapReduce, HDFS,
HBase, and Cassandra). Following the recipe, we easily refactor the
originally problematic configuration to automatically adjust itself and 
delivers
better performance than even the best manually chosen configuration
settings, with little refactoring effort.
Our evaluation shows that, although not a panacea, our control-theory
based recipe can help solve many performance-related configuration problems
in real-world server applications. \shan{need to add some figures for introduction section. maybe move a figure from section 4 here?}



==> tex/note.tex <==
\section{Some notes}

0. System Identification

1. HBASE 5394 \& HBASE 13876 might be used for further experiment

2. What's the challenges?


3. \cite{sironi2013thermos} and \cite{filieri2014automated} are all mainly  deal with lower level goal like energy or temperature, which the variation of system is relative stable.


We need to cite Xray paper \cite{attariyan2012x}.

\cite{xuTooManyKnobs}: (1) the discussion about the Explicit \& Implicit configuration (2) also need cite they categorize the user-reported issues into "difficulties" and "error", an this info is also important. "The difficulties refer to cases where users do not know what or how to configure to obtain their intended system functionalities or performance goals. The errors refer to erroneous settings that caused system misbehavior, such as crashes, hangs, or performance degradation. The users failed to reason out the misconfigurations as the root causes, and thus called support engineers or posted the
problems on online forums and mailing lists. There are other configuration-related issues such as inquiries about general practices and internal usages, categorized as “others.”" (3) performance tuning is hard in house testing (4) HDFS-4618 "That's way too low (I don't know what idiot set it to that.. oh wait, it was me...)"



% about multiple figures



\begin{comment}
\begin{figure*}	
      \begin{minipage}[b]{0.24\linewidth}
			\centering
			\includegraphics
			[width=0.64\textwidth]{fig/blank.pdf}
			\vspace{-4mm}
           \caption{xxx}
           \label{fig:xx}
           \vspace{-1mm}
	   \end{minipage}
	 \hspace{0.1cm}
	\begin{minipage}[b]{0.24\linewidth}
		\centering
		\includegraphics
		[width=0.64\textwidth]{fig/blank.pdf}
		\vspace{-2.5mm}
		\caption {xxx}
		\label{fig:xxx}
		\vspace{-1.7mm}
	\end{minipage}
\end{figure*}
\end{comment}
